New Descriptions of Demazure Tableaux and Right Keys, with Applications to Convexity

The right key of a semistandard Young tableau is a tool used to find Demazure characters for $sl_n(\mathbb{C})$. This thesis gives methods to obtain the right and left keys by inspection of the semistandard Young tableau. Given a partition $\lambda$ and a Weyl group element $w$, there is a semistandard Young tableau $Y_\lambda(w)$ of shape $\lambda$ that corresponds to $w$. The Demazure character for $\lambda$ and $w$ is known to be the sum of the weights of all tableaux whose right key is dominated by $Y_\lambda(w)$. The set of all such tableaux is denoted $\mathcal{D}_\lambda(w)$. Exploiting the method mentioned above for obtaining right keys, this thesis describes the entry at each location in any $T \in \mathcal{D}_\lambda(w)$. Lastly, we will consider $\mathcal{D}_\lambda(w)$ as an integral subset of Euclidean space. The final results present a condition that is both necessary and sufficient for this subset to be convex.

==> zzaareferences.tex <==



\chapter*{References}

\begin{thebibliography}

\bibitem[Av]{}
Aval, J.C.,
      Keys and Alternating Sign Matrices,
      Sem. Lothar. Combin.,
      \textbf{59}, Art. B59f (2008).

\bibitem[Fu]{}
Fulton, W.,
     Young Tableaux,
     London Math. Soc. Student Texts 35,
     Cambridge University Press (1997)

\bibitem[Hu]{}
Humphreys, J.,
    Introduction to Lie Algebras and Representation Theory,
    Springer-Verlag, New York Inc., (1972)

\bibitem[Ko]{}
Kogan, M.,
    Schubert Geometry of Flag Varieties and Gelfan-Cetlin Theory,
    Ph.D. Thesis, M.I.T., June 2000

\bibitem[Ku]{}
Kumar, S.,
     Kac-Moody Groups, their Flag Varieties, and Representation Theory,
     Progress in Mathematics, Volume 204,
     Birkh\"{a}user Boston (2002)


\bibitem[LS]{}
Lascoux, A., and Sch{\"u}tzenberger, M.-P.,
      Keys and Standard Bases,
      Invariant Theory and Tableaux, IMA Volumes in Math and its Applications (D. Stanton, ED.),
      Southend on Sea, UK,
      19 (1990),
      125--144.

\bibitem[Le]{}
Lenart, C.,
     A Unified Approach to Combinatorial Formulas for Schubert Polynomials,
     J. Algebr. Comb.,
     \textbf{20}, (2004),
     263--299

\bibitem[Mac]{}
Macdonald, I.G.,
     Symmetric Functions and Hall Polynomials,
     Oxford Mathematical Monographs,
     Oxford University Press (1979)

\bibitem[Mas]{}
Mason, S.,
     An Explicit Construction of Type A Demazure Atoms,
     J. Algebr. Comb.,
     \textbf{29}, (2009),
     295--313

\bibitem[PS]{}
Postnikov, A. and Stanley, R.,
    Chains in the Bruhat Order,
    J. Algebr. Comb.
    \textbf{29}, (2009),
    133--174

\bibitem[RS]{}
Reiner, V. and Shimozono, M.,
     Key Polynomials and a Flagged {L}ittlewood-{R}ichardson Rule,
     J. Combin. Theory Ser. A
     \textbf{70}, (1995),
      107--143.

\bibitem[St]{}
Stanley, R.,
    Enumerative Combinatorics, Volume 2,
    Cambridge Studies in Advanced Mathematics, Volume 62
    Cambridge University Press (1999)


\bibitem[Wi]{}
Willis, M.,
    A Direct Way to Find the Right Key of a Semistandard Young Tableau,
    arXiv:1110.6184v1 [math.CO]

\end{thebibliography}

